Lifting star-autonomous structures

For a functor $Q$ from a category $C$ to the category $Pos$ of ordered sets and order-preserving functions, we study liftings of various kind of structures from the base category $C$ to the total(or Grothendieck) category $\int Q$. That lifting a monoidal structure corresponds to giving some lax natural transformation making $Q$ almost monoidal, might be part of folklore in category theory.We rely on and generalize the tools supporting this correspondence so to provide exact conditions for lifting symmetric monoidal closed and star-autonomous structures.A corollary of these characterizations is that, if $Q$ factors as a monoidal functor through $SLatt$, the category of complete lattices and sup-preserving functions, then $\int Q$ is always symmetric monoidalclosed. In this case, we also provide a method, based on the double negation nucleus from quantale theory, to turn $\int Q$ into a star-autonomous category.The theory developed, originally motivated from the categories $P-Set$ of Schalk and de Paiva, yields a wide generalization of Hyland and Schalk construction of star-autonomous categories by means of orthogonality structures.

==> corrections.tex <==
\RequirePackage{cancel}
\RequirePackage{ifthen}
\RequirePackage{setspace}
\RequirePackage{xcolor}

\newcommand{\END}{\end{document}}
\newcommand{\TODO}{\red{TODO}\newline}

\newcommand{\added}[1]{\color{blue} #1 \color{black}}
\newcommand{\deleted}[1]{\xcancel{\red{#1}}}
\newcommand{\correction}[2]{\protect\mbox{\xcancel{\red{#1}}~{\blue{#2}}}}

\newcommand{\MathCorrection}[2]{\mbox{$\xcancel{\red{#1}}$\quad{$\blue{#2}$}}}
\newcommand{\TitleCorrection}[2]{\xcancel{\red{#1}}~\blue{#2}}
\newcommand{\commentOut}[2][NON]{
  ~\newline
  \mymarginpar{#1}
  \xcancel{
    \parbox[t]{1.0\linewidth}{
      \begin{minipage}{1.0\linewidth}
        \color{red}
        #2
      \end{minipage}
    }
  }
  \color{black}
  ~\newline
}

\newcommand{\mymarginpar}[1]{\ifthenelse{\equal{#1}{NON}}{}{\marginpar{\vspace{-11mm}\flushleft \setstretch{0.5} \red{\tiny #1}}}}
\newcommand{\bigCorrection}[3][NON]{
  ~\newline
  \mymarginpar{#1}
  \xcancel{
    \parbox[t]{1.0\linewidth}{
      \begin{minipage}{1.0\linewidth}
        \color{red}
        #2
        \color{black}
      \end{minipage}
    }}
  ~\newline
  \parbox[t]{1.0\linewidth}{
    \begin{minipage}{1.0\linewidth}
      \vspace{10mm}
      \color{blue}
      #3
      \color{black}
    \end{minipage}
  }
}


==> macros.tex <==
\RequirePackage{xcolor}
\RequirePackage{tikz}
\RequirePackage{tikz-cd}
\RequirePackage{ebproof}
\RequirePackage{comment}
\RequirePackage{enumerate}
\RequirePackage{mathtools}

\excludecomment{commentout}

\RequirePackage{graphbox}
\RequirePackage{adjustbox}

\RequirePackage{amsmath,amssymb,amsfonts,amsthm}

\RequirePackage{xspace}
\RequirePackage{xcolor}
\RequirePackage{ifthenx}

\RequirePackage{hyperref}
\hypersetup{
  colorlinks=true,
  linkcolor=blue,
  citecolor=blue
}



\input{corrections}


\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\LS}[2][]{\textcolor{red}{LS #1 : #2}}

\newcommand{\CLL}[2][]{\textcolor{purple}{CLL #1 : #2}}
\newcommand{\GC}[2][]{\textcolor{orange}{GC #1 : #2}}
\newcommand{\AFAIRE}{\red{A FAIRE}}
\newcommand{\FINISHSTAT}{\red{TERMINER LA PHRASE ?}}

\newcommand{\RUH}[1][]{\red{#1 Read until here}}

\ifcsl\else
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}[proposition]{Lemma}
\newtheorem{theorem}[proposition]{Theorem}
\newtheorem*{theorem*}{Theorem}
\newcounter{thm}
\renewcommand{\thethm}{\Alph{thm}}
\newtheorem{thmIntro}[thm]{Theorem}

\newtheorem{corollary}[proposition]{Corollary}
\newtheorem{fact}[proposition]{Fact}
\providecommand*\factautorefname{Fact}

\theoremstyle{definition}
\newtheorem{definition}[proposition]{Definition}
\newtheorem*{definition*}{Definition}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{notation}{Notation}
\newtheorem{conjecture}{Conjecture}
\newtheorem{claim}{Claim}
\newtheorem{problem}{Problem}

\newtheoremstyle{exmpl}
{3pt}
{3pt}
{}
{}
{\bf}
{.}
{.5em}
{\thmname{#1}\thmnumber{ #2}\thmnote{: {\bf #3}}}


\newenvironment{Remark}[1][]{\bigskip\ifthenelse{\equal{#1}{}}{\begin{remark}}{\begin{example}[#1]}}{\qedExample\end{remark}}


  \fi
  
  \ifcsl
  \else
  \theoremstyle{exmpl}
  \newtheorem{example}[proposition]{Example}
  \fi
  
\newcommand{\qedExample}{\hfill$\Diamond$}
\RequirePackage{ifthen}

\newenvironment{proofofclaim}{\begin{proof}[Proof of claim]}{\hfill \mbox{(Claim)\qedhere}\end{proof}}

\newenvironment{Example}[1][]{
  \bigskip
  \begin{example}{\ifthenelse{\equal{#1}{}}{}{{\bf #1.}}}}
  {
  \end{example}}


\newtheorem{question}{Question}
\newtheorem{questions}{Questions}


\newcommand{\Myparagraph}[1]{\bigskip\paragraph{\bf #1}}



\newcommand{\trup}[1]{{#1}^{\sharp}}
\newcommand{\Trup}[1]{\trup{(#1)}}
\newcommand{\tr}[1]{\trup{#1}}
\newcommand{\trdown}[1]{{#1}^{\flat}}
\newcommand{\Trdown}[1]{\trdown{(#1)}}
\newcommand{\FUN}{(\,-\,)}
\newcommand{\trupMap}{\trup{\FUN}}
\newcommand{\trdownMap}{\trdown{\FUN}}


\newcommand{\IHom}[1]{[#1]}
\newcommand{\Hom}[1]{\hom(#1)}
\newcommand{\Star}[1]{{#1}^{\ast}}
\newcommand{\STAR}[1]{#1{}^{\ast}}
\newcommand{\SStar}[1]{{#1}\Star{}\Star{}}
\newcommand{\SSStar}[1]{\SStar{#1}{}^{\ast}}
\newcommand{\Perp}[1]{{#1}^{\perp}}
\renewcommand{\Tilde}[1]{\widetilde{#1}}

\newcommand{\HSS}{\IHom{S,S}}

\newcommand{\SI}{\Star{I}}
\newcommand{\SSI}{\SStar{I}}
\newcommand{\SX}{\Star{X}}
\newcommand{\SY}{\Star{Y}}
\newcommand{\SSX}{\SStar{X}}
\newcommand{\SSY}{\SStar{Y}}
\newcommand{\SSSX}{\SSStar{X}}
\newcommand{\SSSY}{\SSStar{Y}}
\newcommand{\HXY}{\IHom{X,Y}}
\newcommand{\HYX}{\IHom{Y,X}}
\newcommand{\HSYSX}{\IHom{\SY,\SX}}
\newcommand{\SM}{\Star{M}}
\newcommand{\SSM}{\Star{M}\Star{}}
\newcommand{\SQ}{\Star{Q}}
\newcommand{\SSQ}{\Star{Q}\Star{}}
\newcommand{\SA}{\Star{A}}
\newcommand{\SSA}{\SStar{A}}
\renewcommand{\SS}{\SStar{}}
\newcommand{\SSS}{\Star{S}\Star{}}
\newcommand{\SB}{\Star{B}}
\newcommand{\SSB}{\SStar{B}}
\newcommand{\SC}{\Star{C}}

\newcommand{\HMM}{\IHom{M,M}}
\newcommand{\HSMSM}{\IHom{\SM,\SM}}

\newcommand{\ev}{\mathtt{ev}}
\newcommand{\trace}{tr}

\newcommand{\rto}[1][\qquad]{\xrightarrow{#1}}
\newcommand{\Rto}[1][\qquad]{\xrightarrow{\;\;#1\;\;}}
\newcommand{\Relto}[1][\qquad]{\dashrightarrow}

\newcommand{\eqdef}{:=}
\newcommand{\defeq}{=:}
\newcommand{\smallLHS}[2][20mm]{\makebox[#1][l]{${\displaystyle #2}$}}
\newcommand{\Gr}{Grothendieck\xspace}
\newcommand{\Gc}{\Gr construction\xspace}

\newcommand{\tor}{\text{or}}
\newcommand{\Tor}{\;\;\tor\;\;}
\newcommand{\tand}{\text{and}}
\newcommand{\Tand}{\;\;\tand\;\;}
\newcommand{\tiff}{\text{iff}}
\newcommand{\Tiff}{\;\;\tiff\;\;}
\newcommand{\Timplies}{\;\;\text{implies}\;\;}
\newcommand{\Tst}{\;\;\tst\;\;}
\newcommand{\tst}{\text{s.t.}}


\newcommand{\C}{\mathsf{C}}
\newcommand{\E}{\mathsf{E}}
\newcommand{\G}{\mathsf{G}}
\newcommand{\B}{\mathsf{B}}
\newcommand{\A}{\mathsf{A}}
\newcommand{\homm}[2]{[#1, #2]} 
\newcommand{\ri}{\operatorname{r}}
\newcommand{\li}{\operatorname{l}}




\newcommand{\tensor}{\otimes}
\newcommand{\stensor}{\widehat{\otimes}}
\newcommand{\tesnor}{\otimes}
\newcommand{\cotensor}{\oplus}
\newcommand{\parr}{\rotatebox[origin=c]{180}{$\mathcal{\&}$}}
\newcommand{\comult}{\parr}
\newcommand{\Bot}{\rotatebox[origin=c]{90}{$\vDash$}}
\newcommand{\Top}{\rotatebox[origin=c]{270}{$\vDash$}}



\newcommand{\bil}[1][\cdot]{\langle#1\rangle}
\renewcommand{\brack}[1]{\bil[#1]}
\newcommand{\bilr}[1][\cdot]{\bil[#1]{}^{\perp}}
\newcommand{\bill}[1][\cdot]{{}^{\perp}\bil[#1]}


\newcommand{\QSet}[1][Q]{\ensuremath{#1\text{-}\mathsf{Set}}\xspace}
\newcommand{\QFSet}[1][Q]{\ensuremath{#1_{F}\text{-}\mathsf{Set}}\xspace}

\newcommand{\Set}{\ensuremath{\mathsf{Set}}\xspace}
\newcommand{\Rel}{\ensuremath{\mathsf{Rel}}\xspace}
\newcommand{\QRel}{\ensuremath{\Rel(Q)}\xspace}

\newcommand{\Map}{\mathsf{Map}}
\newcommand{\SLatt}{\ensuremath{\mathsf{SLatt}}\xspace}
\newcommand{\Nuts}{\ensuremath{\mathsf{Nuts}}\xspace}
\newcommand{\Pos}{\ensuremath{\mathsf{Pos}}\xspace}
\newcommand{\RVect}{\ensuremath{\R\text{-}\mathsf{Vect}}\xspace}
\newcommand{\InfSLatt}{\ensuremath{\mathsf{InfSLatt}}\xspace}
\newcommand{\lrimpl}{\backslash}
\newcommand{\rlimpl}{/}
\newcommand{\lrcoimpl}{\rhd}
\newcommand{\rlcoimpl}{\lhd}

\newcommand{\rneg}[1][(\,\cdot\,)]{{#1}^{\perp}}
\newcommand{\lneg}[1][(\,\cdot\,)]{{}^{\perp}{#1}}
\newcommand{\Rneg}[1]{{#1}{}^{\perp}}
\newcommand{\Dneg}[1]{\Rneg{#1}\Rneg{}}
\newcommand{\Lneg}[1]{{}^{\perp}{#1}}
\newcommand{\Lnegj}[1]{{}^{\perp^{\j}}{#1}}
\newcommand{\Loplus}{\,{}_{\perp}\!\!\oplus}
\newcommand{\Roplus}{\oplus_{\perp}}

\newcommand{\SLTL}{\SL\tensor L}
\newcommand{\LTSL}{L\tensor \SL}
\newcommand{\SLtL}{\SLTL}
\newcommand{\HLL}{\IHom{L,L}}
\newcommand{\HSLSL}{\IHom{\SL,\SL}}


\newcommand{\myqedhere}[1][0mm]{
  \mbox{
    \begin{tabular}[t]{@{\hspace{0mm}}r@{\hspace{0mm}}}
      \\[#1]
      \qedhere
    \end{tabular}
  }
}

\newcommand{\Fsg}{Frobenius semigroup\xspace}
\newcommand{\iso}{\simeq}
\newcommand{\V}{\ensuremath{\mathcal{V}}}

\newcommand{\Rans}[1]{{#1}^{\vee}}
\newcommand{\Rani}[1]{{#1}^{\wedge}}
\newcommand{\rans}[1]{{#1}{}^{\vee}}
\newcommand{\rani}[1]{{#1}{}^{\wedge}}

\newcommand{\rand}[1]{#1\rani{}\rans{}}
\newcommand{\ranD}[1]{#1\rans{}\rani{}}
\newcommand{\Homs}[1]{{\homm{#1}{#1}}_{\vee}}
\newcommand{\LLs}{{\homm{L}{L}}_{\vee}}
\newcommand{\LLi}{{\homm{L}{L}}_{\wedge}}
\newcommand{\LLst}{\LLs^{t}}
\newcommand{\LLit}{\LLi^{t}}
\newcommand{\LLt}{\LLst}

\newcommand{\mix}{\mathtt{mix}}
\newcommand{\SL}{\Star{L}}
\newcommand{\SSL}{\SStar{L}}
\newcommand{\op}{\operatorname{op}}
\newcommand{\Ld}{{L}^{\op}}
\newcommand{\Md}{{M}^{\op}}
\newcommand{\Qd}{{Q}^{\op}}
\newcommand{\SYTX}{\SY\tensor X}


\newcommand{\ifff}{\text{  iff  }}
\newcommand{\Ifff}{\quad\text{iff}\quad}
\newcommand{\contr}{a contradiction\xspace}
\newcommand{\Impl}[2]{(#1) $\Rightarrow$ (#2)}
\newcommand{\ra}{right adjoint\xspace}
\newcommand{\la}{left adjoint\xspace}
\newcommand{\jp}{sup-preserving\xspace}
\renewcommand{\sp}{sup-preserving\xspace}
\newcommand{\ip}{inf-preserving\xspace}
\newcommand{\opr}{order-preserving\xspace}
\renewcommand{\mp}{inf-preserving\xspace}
\newcommand{\LL}{L^{L}}

\newcommand{\funNB}{-}
\newcommand{\fun}{(\funNB)}

\newcommand{\adj}{\dashv}
\newcommand{\rightIso}[1]{\xrightarrow{\,\overset{\raisebox{4pt}{{$\scriptsize
          #1$}}}{\raisebox{-4pt}{$\tiny \sim$}}\,}}
\newcommand{\rIso}[1]{\rightIso{#1}}

\newcommand{\bm}{bracketed magma\xspace}
\newcommand{\abm}{associative bracketed magma\xspace}
\newcommand{\id}{\mathtt{id}}

\newcommand{\lact}[1][A]{\alpha^{\ell}_{#1}}
\newcommand{\ract}[1][B]{\alpha^{\rho}_{#1}}
\newcommand{\affine}{affine\xspace}
\newcommand{\pseudoaffine}{pseudo-affine\xspace}
\newcommand{\paffine}{\pseudoaffine}


\newcounter{useDiagCount}
\setcounter{useDiagCount}{0}
\newcommand{\useDiagram}[2][]{
  \ifthenelse{\isinteger{#1}}{
    \setcounter{useDiagCount}{#1}
    \includegraphics[page=#1,align=c]{#2}
  }{
    \stepcounter{useDiagCount}
    \def\page{\theuseDiagCount}
    \includegraphics[page=\page,align=c,#1]{#2}
  }
}

\newcommand{\cl}{complete lattice\xspace}
\newcommand{\cd}{completely distributive\xspace}
\newcommand{\cdlatt}{\cd lattice\xspace}
\newcommand{\upTensor}{\widehat{\tensor}}
\newcommand{\RT}{Raney's theorem\xspace}

\newcommand{\set}[1]{\{ \,#1\,\}}
\newcommand{\downset}[1]{\downarrow #1}
\newcommand{\Downset}[2][X]{\,\downarrow_{#1}\!\!(#2)}
\newcommand{\two}{\mathbf{2}}
\newcommand{\closure}[1]{\overline{#1}}
\newcommand{\positive}{positive\xspace}
\newcommand{\strong}{strongly continuous\xspace}

\newcommand{\card}[1]{|#1|}

\newcommand{\leftA}{l}
\newcommand{\rightA}{r}
\newcommand{\leftB}{\leftA^{-1}}
\newcommand{\rightB}{\rightA^{-1}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\pairing}[1]{\langle#1\rangle}
\newcommand{\Pairing}[1]{(#1)}
\newcommand{\innerH}[1]{\pairing{#1}_{H}}
\newcommand{\normH}[1]{||#1||_{H}}

\newcommand{\qmult}{\ast}
\newcommand{\Cstar}{\ensuremath{\mathrm{C}^{\ast}}}

\renewcommand{\SM}{symmetric monoidal\xspace}
\newcommand{\SMC}{symmetric monoidal closed\xspace}
\newcommand{\SMCC}{\SMC category\xspace}
\newcommand{\aut}{autonomous\xspace}
\newcommand{\saut}{$\ast$-autonomous\xspace}
\newcommand{\sautcat}{\saut category\xspace}
\newcommand{\sautcats}{\saut categories\xspace}
\newcommand{\autcat}{autonomous category\xspace}
\newcommand{\autcats}{autonomous categories\xspace}
\newcommand{\chu}{\operatorname{Chu}_{\V,\zero}}
\newcommand{\Pair}{\operatorname{Pair}_{\V,\zero}}
\newcommand{\Ens}{\mathbf{Set}}
\newcommand{\sem}[1]{{\textbf{Sem}}_{#1}}
\newcommand{\vect}{\textbf{Vect}}
\newcommand{\cat}{category\xspace}
\newcommand{\cats}{categories\xspace}
\newcommand{\I}{\mathcal{I}}

\newcommand{\radj}[1]{\rho(#1)}
\newcommand{\ladj}[1]{\ell(#1)}
\newcommand{\cotight}{cotight\xspace}


\newcommand{\pr}[1]{\operatorname{pr}_{#1}}


\newcommand{\zero}{0}
\newcommand{\SATA}{\SA\tensor A}
\newcommand{\HAA}{\IHom{A,A}}
\newcommand{\HXX}{\IHom{X,X}}
\newcommand{\frob}{(A,B,\epsilon,\mu_A, \leftA,\rightA)}






\newcommand{\Gammaempt}{\Gamma^{\emptyset}}
\newcommand{\Deltaempt}{\Delta^{\emptyset}}

\newcommand{\conv}{\mathtt{c}}
\newcommand{\impl}{\multimap}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\gen}[1]{\langle #1\rangle}

\newcommand{\Fs}{Frobenius structure\xspace}
\newcommand{\Zp}{\mathcal{Z}^{+}}
\newcommand{\Zpu}{\Zp_{u}}
\newcommand{\lad}{\dashv}
\newcommand{\IMPL}{\multimap}
\newcommand{\transpose}[1]{{#1}^{\sharp}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\Rp}{\R_{+}}
\newcommand{\abs}[1]{| #1 |}
\newcommand{\norm}[2][]{|| #2 ||_{#1}}
\newcommand{\N}{\mathcal{N}}

\newcommand{\FD}{\mathcal{F}_\mathtt{d}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\U}{\mathcal{U}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\UP}{\U\P}
\newcommand{\EQ}[1][Q]{\mathtt{E}_{#1}}

\newcommand{\cod}{\mathrm{cod}}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\Obj}{\mathsf{Obj}}
\newcommand{\upset}{\uparrow}
\newcommand{\singlel}{\ast}
\newcommand{\singleton}{\set{\singlel}}
\newcommand{\iQ}{\int Q}
\newcommand{\lift}[1]{\overline{#1}}
\newcommand{\lent}{lax extranatural transformation\xspace}
\newcommand{\lF}{\lift{F}}
\newcommand{\setof}[1][n]{[#1]}


\newenvironment{blue}{\color{blue}}{\color{black}}
\newcommand{\talpha}{\widetilde{\alpha}}
\newcommand{\tbeta}{\widetilde{\beta}}
\newcommand{\wt}[1]{\widetilde{#1}}

\newcommand{\nn}[1][q]{\neg\neg_{#1}}
\newcommand{\nno}{\nn[\omega]}
\renewcommand{\j}{\jmath^{\omega}}

\newcommand{\Qj}{Q^{\j}}

\newcommand{\supj}{\bigsqcup}
\newcommand{\bigveej}{\supj}

\newcommand{\muj}{\mu^{\j}}
\newcommand{\uj}{u^{\j}}
\renewcommand{\brack}[2][]{\langle #2 \rangle^{#1}}
\newcommand{\brackj}[1]{\brack[\j]{#1}}
\newcommand{\brackfun}{\brack{\cdot,\cdot}}
\newcommand{\omegaj}{\omega^{\j}}

\newcommand{\SdP}{Schalk and de Paiva\xspace}
\newcommand{\HS}{Hyland and Schalk\xspace}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\OCorth}{{\cal O}_{\independent}{(\C)}}

\DeclareMathOperator{\alg}{Alg}
\DeclareMathOperator{\coalg}{CoAlg}


\newcommand{\ucq}{unital commutative quantale\xspace}


\newcommand{\ie}{\textit{i.e.}\xspace}

\newcommand{\eg}{\textit{e.g.}\xspace}

\newcommand{\etc}{\textit{e.t.c.}\xspace}



\newcommand{\final}{terminal\xspace}

\newcommand{\Qnu}{Q^{\nu}}
\newcommand{\Qmu}{Q^{\mu}}

\newcommand{\QS}{\Star{Q}}
\newcommand{\QSnu}{\QS{}^{\nu}}
\newcommand{\QSnuS}{\QSnu\Star{}}

\newcommand{\within}[2][\quad]{\quad \text{in $#2$}#1} 

\newcommand{\cal}[1]{\mathcal{#1}}


